Achieving Perfect Location Privacy in Wireless Devices Using Anonymization

The popularity of mobile devices and location-based services (LBS) has created great concern regarding the location privacy of their users. Anonymization is a common technique that is often used to protect the location privacy of LBS users. Here, we present an information-theoretic approach to define the notion of perfect location privacy. We show how LBS's should use the anonymization method to ensure that their users can achieve perfect location privacy. First, we assume that a user's current location is independent from her past locations. Using this i.i.d model, we show that if the pseudonym of the user is changed before $O(n^{\frac{2}{r-1}})$ observations are made by the adversary for that user, then the user has perfect location privacy. Here, n is the number of the users in the network and r is the number of all possible locations that users can go to. Next, we model users' movements using Markov chains to better model real-world movement patterns. We show that perfect location privacy is achievable for a user if the user's pseudonym is changed before $O(n^{\frac{2}{|E|-r}})$ observations are collected by the adversary for the user, where |E| is the number of edges in the user's Markov chain model.

==> markovchain.tex <==
\section{Markov Chain Model}
Assume there are $r$ possible locations that users can go to. We use a Markov chain ($MC$) with $r$ states to model movements of each user, Figure~\ref{mc}. We define $E$, the set of edges in this Markov chain such that $(i,j)$ is in $E$ if there exists an edge from $i$ to $j$ with probability $p{(i,j)}>0$.

\begin{figure}[H]
\begin{center}
\[
\SelectTips {lu}{12 scaled 1500}
\xymatrixcolsep{3pc}\xymatrixrowsep{3pc}\xymatrix{
*++[o][F-]{1}  \ar@(dl,ul)[]^{p(1,1)} \ar@/^1pc/[r]^{p(1,2)}
&*++[o][F-]{2}
\\ *++[o][F-]{3} \ar@/^/[u]_{p(3,1)} &\cdots
&*++[o][F-]{r} \ar@/^/[ul]_{p(r,2)}  \ar@/^/[ull]_{p(r,1)}
}
\]
\caption{Markov chain model $MC$ with $r$ states and $|E|$ edges.}
\label{mc}
\end{center}
\end{figure}
We assume that this Markov chain gives the movement pattern of each user and what differentiates between users is their transition probabilities. That is, for fixed locations $i$ and $j$, two different users could have two different transition probabilities.


%We now state and prove the main Theorem that gives the condition for perfect location privacy for a user in the above setting.
\begin{thm}\label{main}
For an irreducible, aperiodic Markov chain with $r$ states and $|E|$ edges, if $m = cn^{\frac{2}{|E|-r}-\alpha}$, where $c>0$ and $\alpha>0$ are constants, then
\begin{align}
\lim_{n \rightarrow \infty}{I(X_1(k) ; \textbf{Y}^{(m)})} = 0,\ \ \ \forall k \in \mathbb{N},
\end{align}
i.e., user 1 has perfect location privacy.
\end{thm}

\begin{proof}

First note that since the Markov chain is irreducible and aperiodic, when we are determining $p(i,j)$'s, there are $d$ degrees of freedom, where $d$ is equal to $|E| - r$. This is because for each states $i$, we must have
\begin{align}
\no \sum \limits_{j = 1}^{r} p(i,j) = 1.
\end{align}
Thus, the Markov chain of the user $u$ is completely determined by $d$ values of $p(i,j)$'s which we show them as
\begin{align}
\no \textbf{P}_{u} = \left(p_u(1),p_u(2),\cdots,p_u(d)\right)
\end{align}
and $\textbf{P}_{u}$'s are known to the adversary for all users. Note that the choice of $\textbf{P}_{u}$ is not unique; nevertheless, as long as we fix a specific $\textbf{P}_{u}$, we can proceed with the proof.
We define $E_d$ as the set of $d$ edges whose $p(i,j)$'s belong to  $\textbf{P}_{u}$. Let $R_{\textbf{p}} \subset \mathbb{R}^{d}$ be the range of acceptable values for $\textbf{P}_{u}$. For example, in Figure \ref{ex1} we have $|E|=6$ and $r=3$, so we have three independent transitions probabilities. If we choose $p_1$, $p_2$ and $p_3$ according to the figure, we obtain the following region
\begin{align}
\no R_{\textbf{p}} =\{(p_1,p_2,p_3)  \in \mathbb{R}^3: 0 \leq p_i \leq 1 \textrm{ for } i = 1,2,3 \textrm{ and } p_1 + p_2 \leq 1\}.
\end{align}

\begin{figure}[H]
\begin{center}
\[
\SelectTips {lu}{12 scaled 1500}
\xymatrixcolsep{5pc}\xymatrixrowsep{5pc}\xymatrix{
*++[o][F-]{1}  \ar@(dl,ul)[]^{p_1}\ar@/^/[r]^{p_2}  \ar@/^0.7pc/[dr]|{1-p_1-p_2}
& *++[o][F-]{2} \ar@/^1pc/[d]^{1}
\\ & *++[o][F-]{3}  \ar@/^/[u]_{p_3}  \ar@/^1.2pc/[ul]|{1-p_3}
}
\]
\caption{Three states Markov chain example}
\label{ex1}
\end{center}
\end{figure}
The statistical properties of each user are completely known to the adversary since he/she knows the Markov chain of each user. The adversary wants to be able to distinguish between users by having $m$ observations per user and also knowing $\textbf{P}_{u}$'s for all users.

In this model, we assume that $\textbf{P}_{u}$ for each user $u$ is drawn independently from a $d$-dimensional continuous density function, $f_{\textbf{P}}(\textbf{p})$. As before, we assume there exist positive constants $ \delta_1,\delta_2>0$, such that
\begin{equation}
\begin{cases}
\no    \delta_1 <f_{\textbf{P}}(\textbf{p}) <\delta_2 & \textbf{p} \in R_{\textbf{p}}\\
    f_{\textbf{P}}(\textbf{p})=0 &  \textbf{p} \notin R_{\textbf{p}}
\end{cases}
\end{equation}

We now claim that the adversary's position in this problem is mathematically equivalent to the the i.i.d model where the number of locations $r$ is equal to $d+1$ where $d = |E|-r$. First, note that since the Markov chain is irreducible and aperiodic, it has a unique stationary distribution which is equal to the limiting distribution. Next, define $\mathbf{Q}_u$ to be the vector consisting of all the transition probabilities of user $u$. In particular, based on the above argument, we can represent $\mathbf{Q}_u$ in the following way:
\begin{align}
\no \mathbf{Q}_u=[\mathbf{P}_{u}, \mathbf{P}_{u} \mathbf{B}],
\end{align}
where $\mathbf{B}$ is a non-random $d$ by $|E|-d$ matrix. Now, note that $\mathbf{P}_{u} \mathbf{B}$ is a non-random function of $\mathbf{P}_{u}$. In particular, if $M_u(i,j)$ shows the observed number transitions from sate $i$ to state $j$ for user $u$, then we only need to know $M_u(i,j)$ for the edges in $E_d$ as the rest will be determined by the linear transform defined by $\mathbf{B}$. This implies that the decision problem for the adversary is reduced to the decision problem on transition probabilities in $\mathbf{P}_{u}$ and the adversary only needs to look at the $M_u(i,j)$'s for the edges in $E_d$. Now, this problem has exactly the same structure as the i.i.d model where the number of locations $r$ is equal to $d+1$ where $d = |E|-r$. In particular, $M_u(i,j)$'s have multinomial distributions and the statement of Theorem \ref{main} follows by applying Theorem \ref{r_state_thm}.

\end{proof}



\textit{Discussion:} One limitation of the above formulations is that all users must have the same Markov chain graphs with only different transition probabilities. In reality, there might be users that have different Markov chain graphs. For example, we might have users that never visit a specific region. Nevertheless, we can address this issue in the following way. If we are considering the location privacy of user $1$, we only consider users that have the same Markov chain graph (but with different transitions probabilities). The other users are easily distinguishable from user $1$ anyway. Now, $n$ would be the total number of this new set of users and again we can apply Theorem~\ref{main}. If $n$ is not large enough in this case, then we need to use location obfuscation techniques in addition to anonymization to achieve perfect privacy.

